Classification of degenerate non-homogeneous Hamiltonian operators

In this paper, the authors investigate non-homogeneous Hamiltonian operators composed of a first-order Dubrovin-Novikov operator and an ultralocal one. The study of such operators turns out to be fundamental for the inverted system of equations associated with a class of Hamiltonian scalar equations. Often, the involved operators are degenerate in the first-order term. For this reason, a complete classification of the operators with degenerate leading coefficient in systems of 2 and 3 components is presented.

==> biblio_old.tex <==

\begin{thebibliography}{10}
\bibitem{AgaFer}
S. I . Agafonov and E. V. Ferapontov,
\newblock \emph{Systems of conservation laws in the context of the projective theory of congruences},
\newblock Izv. RAN. Ser. Mat., 1996, Volume 60, Issue 6, Pages 3–30.

\bibitem{dorfman91:_local}
I.Ya. Dorfman and O.I. Mokhov.
\newblock Local symplectic operators and structures related to them.
\newblock {\em J. Math. Phys.}, 32:3288, 1991.


\bibitem{dubrovin89} 
B. A. Dubrovin: \emph{Differential-geometric Poisson brackets on a lattice}, 1989, 131-133, 23:2,Functional Analysis and Its Applications.

\bibitem{DubKri} B. A. Dubrovin, I. M. Krichever, and S. P. Novikov.
\newblock  Integrable systems. I. In \emph{Dynamical Systems IV}, volume 4 of Encyclopaedia of Mathematical Sciences, 
\newblock pages 173–280. Springer-Verlag, Berlin, 2 edition, 2001.

\bibitem{DN83}
B.A. Dubrovin and S.P. Novikov:
\newblock \emph{Hamiltonian formalism of one-dimensional systems of hydrodynamic type
  and the Bogolyubov--Whitham averaging method}.
\newblock {\em Soviet Math. Dokl.}, 27(3):665--669, 1983.

\bibitem{DubrovinNovikov:PBHT}
B.~A. Dubrovin and S.~P. Novikov:
\newblock \emph{Poisson brackets of hydrodynamic type}.
\newblock {\em Soviet Math. Dokl.}, 30:651--654, 1984.




\bibitem{falq}
G. Falqui:
\newblock \emph{On a Camassa-Holm type equation with two dependent variables}, 
\newblock J. Phys. A.: Math. Gen. 39(2006),327-342.

\bibitem{FerKar} Ferapontov, E.V., Khusnutdinova, K.R.: On integrability of (2+1)-dimensional quasilinear systems.
Commun. Math. Phys. 248, 187–206 (2004)

\bibitem{FeraMarshall}
E.V. Ferapontov, D. Marshall:
   \emph{Differential-geometric approach to the integrability of hydrodynamic chains: the Haantjes tensor}, Math. Ann., 339, 2007.
   
\bibitem{Mor} E. Ferapontov, A. Moro, V. Sokolov (2008) Hamiltonian systems of hydrodynamic type in 2+1
dimensions. Commun. Math. Phys. Vol. 285, pp. 31-65.

\bibitem{FPV14}
E.V. Ferapontov, M.V. Pavlov, and R.F. Vitolo:
\newblock \emph{Projective-geometric aspects of homogeneous third-order {H}amiltonian
  operators}.
\newblock {\em J. Geom. Phys.}, 85:16--28, 2014.
\newblock \texttt{DOI:10.1016/j.geomphys.2014.05.027}.

\bibitem{FerPavVit1} E. V. Ferapontov, M. V. Pavlov and R. Vitolo:
\newblock \emph{Systems of conservation laws with third-order Hamiltonian structures}, 
\newblock Lett. Math. Phys. 108, Issue 6 (2018), 1525-1550.




%\bibitem{Getzler:DTHOpFCV}
%E.~Getzler.
%\newblock A {D}arboux theorem for {H}amiltonian operators in the formal
%  calculus of variations.
%\newblock {\em Duke Math. J.}, 111:535--560, 2002.

%\bibitem{haantjes55:_x}
%J.~Haantjes.
%\newblock On $x_m$-forming sets of eigenvectors.
%\newblock {\em Indag. Math.}, 17:158--162, 1955.

%\bibitem{Ibragimov:NCT}
%N.~H. Ibragimov.
%\newblock A new conservation theorem.
%\newblock {\em J. Math. Anal. Appl.}, 333:311--328, 2007.

%\bibitem{KrasilshchikKersten:SROpCSDE}
%I.~S. Krasil{\cprime}shchik and P.~H.~M. Kersten.
%\newblock {\em Symmetries and Recursion Operators for Classical and
%  Supersymmetric Differential Equations}.
%\newblock Kluwer, 2000.

\bibitem{hampds} P. Kersten, I.S. Krasil'shchik, A.M. Verbovetsky, R. Vitolo: \emph{Hamiltonian structures for general PDEs},
in B. Kruglikov, V. Lychagin, E. Straume: Differential Equations – Geometry, Symmetries and Integrability, Proceedings of the 2008 Abel Symposium, Springer, 187–198.

\bibitem{KerstenKrasilshchikVerbovetsky:HOpC}
P.~Kersten, I.~Krasil'shchik, and A.~Verbovetsky.
\newblock Hamiltonian operators and $\ell^*$-coverings.
\newblock {\em J. Geom. Phys.}, 50:273--302, 2004.

\bibitem{koinho} A. Konyaev: \emph{Geometry of inhomogeneous Poisson brackets, multicomponent Harry Dym hierarchies and multicomponent Hunter-Saxton equations}, preprint, arXiv:2112.05635

\bibitem{KVV17}
J.~Krasil'shchik, A.~Verbovetsky, and R.~Vitolo:
\newblock {\em The symbolic computation of integrability structures for partial
  differential equations}.
\newblock Texts and Monographs in Symbolic Computation. Springer, 2018.
\newblock ISBN 978-3-319-71654-1; see \url{http://gdeq.org/Symbolic_Book} for
  downloading program files that are discussed in the book.

%\bibitem{KV11}
%J.~Krasil{\cprime}shchik and A.~M. Verbovetsky.
%\newblock Geometry of jet spaces and integrable systems.
%\newblock {\em J. Geom. Phys.}, 61:1633--1674, 2011.
%\newblock arxiv:1002.0077.

\bibitem{LSV:bi_hamil_kdv}
P.~Lorenzoni, A.~Savoldi, and R.~Vitolo:
\newblock \emph{{B}i-{H}amiltonian systems of {KdV} type}.
\newblock {\em J. Phys. A}, 51(4):045202, 2018.

\bibitem{Magri:SMInHEq}
F.~Magri:
\newblock \emph{A simple model of the integrable {H}amiltonian equation}.
\newblock {\em J. Math. Phys.}, 19:1156--1162, 1978.

%\bibitem{MalNov2001}
%A.Ya. Maltsev and S.P. Novikov.
%\newblock On the local systems {H}amiltonian in the weakly non-local {P}oisson
%  brackets.
%\newblock {\em Phys.\ D}, 156(1-2):53--80, 2001.
\bibitem{FerMok1}
O. I. Mokhov, E. V. Ferapontov, 
\newblock \emph{Hamiltonian Pairs Associated with Skew-Symmetric Killing Tensors on Spaces of Constant Curvature}.
\newblock Funktsional. Anal. i Prilozhen., 28:2 (1994), 60–63; Funct. 
Anal. Appl., 28:2 (1994), 123–125.

\bibitem{mokhov98:_sympl_poiss}
O.I. Mokhov.
\newblock \emph{Symplectic and {P}oisson geometry on loop spaces of smooth manifolds
  and integrable equations}.
  
 \bibitem{mk2} O.I. Mokhov 1990 Russ. Math. Surv. 45 218
\newblock In S.P. Novikov and I.M. Krichever, editors, {\em Reviews in
  mathematics and mathematical physics}, volume~11, pages 1--128. Harwood
  academic publishers, 1998.



\bibitem{NovikovManakovPitaevskiiZakharov:TS}
S.~P. Novikov, S.~V. Manakov, L.~P. Pitaevskii, and V.~E. Zakharov:
\newblock {\em Theory of Solitons}.
\newblock Plenum Press, 1984.

%\bibitem{olver88:_darboux_hamil}
%P.~Olver.
%\newblock Darboux' theorem for hamiltonian differential operators.
%\newblock {\em J. Differential Equations}, 71:10--33, 1988.
\bibitem{Olver:ApLGDEq}
P.J. Olver:
\newblock {\em Applications of {L}ie Groups to Differential Equations}.
\newblock Springer-Verlag, 2nd edition, 1993.

\bibitem{harry_dym_bi_hamiltonian}
Pedroni, M., Sciacca, V. and Zubelli, J.: \emph{On the Bi-Hamiltonian Theory for the Harry Dym Equation}, 133Theoretical and Mathematical Physics, 2002.


\bibitem{sav1} A. Savoldi: \emph{On deformations of one-dimensional Poisson structures of hydrodynamic type with degenerate metric}, J. Geom. Phys 104 (2016), pp. 246–276.

\bibitem{tsa3} S.P. Tsarev: \emph{The hamiltonian property of stationary and inverse equations of condensed matter mechanics and mathematical physics}. Math. Notes 46, 569–573 (1989)

\bibitem{tsarev85:_poiss_hamil}
S.P.~Tsarev:
\newblock \emph{On {P}oisson brackets and one-dimensional {H}amiltonian systems of
  hydrodynamic type}.
\newblock {\em Soviet Math. Dokl.}, 31(3):488--491, 1985.

\bibitem{tsarev91:_hamil}
S.P. Tsarev:
\newblock \emph{The geometry of {H}amiltonian systems of hydrodynamic type. the
  generalized hodograph method}.
\newblock {\em Math. USSR-Izv.}, 37(2):397--419, 1991.

\bibitem{VerVit1}
P. Vergallo and R. Vitolo: \emph{Homogeneous Hamiltonian operators and the theory of coverings},
\newblock Differential Geom. Appl., 75:101713, 2021, arXiv: \url{https://arxiv.org/abs/2007.15294}.

 \bibitem{VerVit2}
P. Vergallo and R. Vitolo:
\newblock \emph{Projective geometry of homogeneous second order Hamiltonian operators},
\newblock {\em arXiv}, \url{https://arxiv.org/abs/2203.04237}, March 2022.


 

%\bibitem{vinogradov84:_categ}
%A.M. Vinogradov.
%\newblock Category of partial differential equations.
%\newblock {\em Lecture {N}otes in {M}ath.}, 1108:77--102, 1984.
%\newblock Springer-Verlag, Berlin.


\bibitem{Vit1}
R. Vitolo:
\newblock \emph{Computing with Hamiltonian operators},
\newblock Computer Physics 
Communications Volume 244 (2019), 228-245.
\end{thebibliography}
